Quantifying Surface Heterogeneity Across Asteroid (101955) Bennu using Candidate Site Remote Sensing Data

The OSIRIS-REx mission acquired spatially resolved (2-10 m spot sizes) visible-near infrared (VNIR) and thermal infrared (TIR) spectra across four candidate sampling sites on asteroid (101955) Bennu: Nightingale, Osprey, Sandpiper, and Kingfisher. To quantify heterogeneity across a small body (about 500 m radius) like Bennu, we explore remotely observed spectral data to draw conclusions about the mineralogical composition and key physical processes that drive surface variability. We derive diagnostic band parameters from the OSIRIS-REx Visible and Infrared Spectrometer and the OSIRIS-REx Thermal Emission Spectrometer datasets to quantify compositional and physical variability across sites and assess their mineralogical context. The VNIR spectra exhibit similar overall reflectance shapes but systematic differences in spectral slopes and the 2.74 micron OH absorption. TIR emissivity spectra reveal modest but statistically significant shifts in the Christiansen Feature, silicate stretching, and bending band positions, indicating differences in silicate composition, hydration state, and Mg/Fe relative abundance. Principal component analysis separates each site into distinct clusters in multivariate band-parameter space, whereas K-means clustering identifies intra-site spectral sub-populations. Welch's Analysis of Variance and Hotelling's tests confirm that band-parameter variations between sites are significant. These results reveal that Bennu's surface preserves measurable spectral heterogeneity at 2-10 m scales, with site-to-site variations in hydration indicators and silicate band positions. The spectral properties of Nightingale encompass the full range observed across all four sites, establishing a remote sensing baseline for contextualizing laboratory analyses of the returned sample within Bennu's broader composition diversity and alteration history.

==> anova.tex <==
\section{ANOVA Assumptions}
\label{anova}

Levene's test results for all band parameters are given in Table~\ref{tab:levene}; Welch's ANOVA results replacing the standard one-way ANOVA are given in Table~\ref{tab:welch_anova}. Q-Q plots of within-group residuals are shown in Figure~\ref{fig:qq}.

\begin{table}[htbp]
\centering
\caption{Levene's test for homogeneity of variance across the four
candidate sampling sites for each spectral band parameter.
Parameters with $p < 0.05$ are heteroscedastic; those were re-examined
with Welch's one-way ANOVA (Table~\ref{tab:welch_anova}).}
\label{tab:levene}
\begin{tabular}{llccc}
\hline
Instrument & Parameter & $F$ & $p$-value & Homoscedastic? \\
\hline
\multicolumn{5}{l}{\textit{OVIRS}} \\
& BD$_{0.55}$ & $659.36$ & $< 10^{-300}$ & \textbf{No} \\
& BD$_{1.05}$ & $1001.70$ & $< 10^{-300}$ & \textbf{No} \\
& BD$_{1.40}$ & $606.68$ & $< 10^{-300}$ & \textbf{No} \\
& BD$_{1.80}$ & $939.13$ & $< 10^{-300}$ & \textbf{No} \\
& BD$_{2.74}$ & $785.48$ & $< 10^{-300}$ & \textbf{No} \\
& Spectral Slope & $318.06$ & $3.12 \times 10^{-203}$ & \textbf{No} \\
\hline
\multicolumn{5}{l}{\textit{OTES}} \\
& CF Position (cm$^{-1}$) & $229.02$ & $2.40 \times 10^{-146}$ & \textbf{No} \\
& Spectral Slope & $96.24$ & $6.96 \times 10^{-62}$ & \textbf{No} \\
& Reststrahlen Stretch (cm$^{-1}$) & $26.37$ & $5.10 \times 10^{-17}$ & \textbf{No} \\
& Reststrahlen Bend (cm$^{-1}$) & $250.14$ & $1.18 \times 10^{-159}$ & \textbf{No} \\
\hline
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\caption{Welch's one-way ANOVA for spectral band parameters that
failed Levene's test ($p < 0.05$). Degrees of freedom use the
Welch--Satterthwaite approximation.}
\label{tab:welch_anova}
\begin{tabular}{llcccc}
\hline
Instrument & Parameter & $F$ & $df_1$ & $df_2$ & $p$-value \\
\hline
\multicolumn{6}{l}{\textit{OVIRS}} \\
& BD$_{0.55}$ & $208.68$ & $3$ & $12588.7$ & $1.11 \times 10^{-16}$ \\
& BD$_{1.05}$ & $252.19$ & $3$ & $12810.3$ & $1.11 \times 10^{-16}$ \\
& BD$_{1.40}$ & $16.34$ & $3$ & $12176.4$ & $1.35 \times 10^{-10}$ \\
& BD$_{1.80}$ & $573.85$ & $3$ & $12860.7$ & $1.11 \times 10^{-16}$ \\
& BD$_{2.74}$ & $727.45$ & $3$ & $11314.3$ & $1.11 \times 10^{-16}$ \\
& Spectral Slope & $509.83$ & $3$ & $11532.8$ & $1.11 \times 10^{-16}$ \\
\hline
\multicolumn{6}{l}{\textit{OTES}} \\
& CF Position (cm$^{-1}$) & $314.67$ & $3$ & $8280.5$ & $1.11 \times 10^{-16}$ \\
& Spectral Slope & $728.73$ & $3$ & $9015.9$ & $1.11 \times 10^{-16}$ \\
& Reststrahlen Stretch (cm$^{-1}$) & $339.57$ & $3$ & $8460.8$ & $1.11 \times 10^{-16}$ \\
& Reststrahlen Bend (cm$^{-1}$) & $285.99$ & $3$ & $9649.4$ & $1.11 \times 10^{-16}$ \\
\hline
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{anova_qq_plots.png}
    \caption{ANOVA Q-Q Plots}
    \label{fig:qq}
\end{figure}
